Thermal and Vibrationally Activated Decomposition of the syn-CH$_3$CHOO Criegee Intermediate

The full reaction pathway between the syn-CH$_3$CHOO Criegee Intermediate via vinyl hydroxyperoxide to OH+CH$_2$COH is followed for vibrationally excited and thermally prepared reactants. The rates from vibrational excitation are consistent with those found from experiments and tunneling is not required for reactivity at all initial conditions probed. For vibrationally excited reactant, VHP accumulates and becomes a bottleneck for the reaction. The two preparations - relevant for laboratory studies and conditions in the atmosphere - lead to a difference of close to one order of magnitude in OH production (~ 5 % vs. 35 %) on the 1 ns time scale which is an important determinant for the chemical evolution of the atmosphere.

==> cri(1)/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
